Disentangling Hype from Practicality: On Realistically Achieving Quantum Advantage

Quantum computers offer a new paradigm of computing with the potential to vastly outperform any imagineable classical computer. This has caused a gold rush towards new quantum algorithms and hardware. In light of the growing expectations and hype surrounding quantum computing we ask the question which are the promising applications to realize quantum advantage. We argue that small data problems and quantum algorithms with super-quadratic speedups are essential to make quantum computers useful in practice. With these guidelines one can separate promising applications for quantum computing from those where classical solutions should be pursued. While most of the proposed quantum algorithms and applications do not achieve the necessary speedups to be considered practical, we already see a huge potential in material science and chemistry. We expect further applications to be developed based on our guidelines.

==> Makefile <==
DOCUMENT=$(shell ls -1 *tex | sed -e "s/\.tex//")

FILES=*.tex 

all: $(DOCUMENT).pdf

$(DOCUMENT).pdf: $(FILES)
	if [ -f plt/Makefile ]; then make -C plt; fi
	if [ -f img/Makefile ]; then make -C img; fi
	if [ -d ../img ]; then make -C ../img; fi
	rm -f pdflatex.out
#	cd ppt && sh ./crop_all.sh
	pdflatex --shell-escape $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	if grep -q citation $(DOCUMENT).aux; then bibtex $(DOCUMENT); fi;
# don't use pdflatex due to transparency issues  
	pdflatex --shell-escape $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	pdflatex --shell-escape $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	#dvips $(DOCUMENT).dvi -o $(DOCUMENT).ps
# use ps2pdf to avoid lossy image compression in pdf which looks ugly on the
# beamer
	#ps2pdf14 -dPDFSETTINGS=/printer -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode $(DOCUMENT).ps

copyin: ~/projekte/latex/macros/*
	cp ~/projekte/latex/macros/bibliography.bib .
	cp ~/projekte/latex/macros/htor.sty .
	cp ~/projekte/latex/macros/htor_paper.cls .

show: $(DOCUMENT).pdf
	atril $(DOCUMENT).pdf

spell:
	ln -sf ~/projekte/templates/aspell.en_US.dic .
	for i in $$(ls -1 *.tex); do \
		echo "checking $$i ... "; \
		aspell -t --lang=en_US --home-dir="$$(pwd)" -p aspell.en_US.dic -c $$i; \
done; \

force:
	touch $(DOCUMENT).tex
	make $(DOCUMENT).pdf

clean:
	if [ -f plt/Makefile ]; then make -C plt clean; fi
	rm -f *.aux *.out sparsity.synctex.gz
	rm -f $(DOCUMENT).blg $(DOCUMENT).dvi $(DOCUMENT).vrb comment.cut 
	rm -f $(DOCUMENT).pdf $(DOCUMENT).toc $(DOCUMENT).lo[a,f,g,h,l,t]
	rm -f $(DOCUMENT).nav $(DOCUMENT).snm $(DOCUMENT).ps $(DOCUMENT).out
	rm -f aspell*dic
	if [ -f plt/Makefile ]; then make -C plt clean; fi
	if [ -d img ]; then make -C img clean; fi
	if [ -d slides ]; then make -C img clean; fi
	if [ -d ../img ]; then make -C ../img clean; fi

pack: $(DOCUMENT).tgz

$(DOCUMENT).tgz: *.tex
	mkdir $(DOCUMENT) 
	cp *.tex $(DOCUMENT)
	cp *.bib $(DOCUMENT)
	cp *.bbl $(DOCUMENT)
	cp poster*pdf $(DOCUMENT)
	if [ -d img ]; then cp -a img $(DOCUMENT); fi
	if [ -d kivio ]; then cp -a kivio $(DOCUMENT); fi
	cp Makefile $(DOCUMENT)
	make -C $(DOCUMENT)
	cp $(DOCUMENT)/$(DOCUMENT).pdf $(DOCUMENT)/$(DOCUMENT)_orig.pdf
	make -C $(DOCUMENT) clean
	tar czf $(DOCUMENT).tgz $(DOCUMENT) --exclude=.svn 
	tar tzf $(DOCUMENT).tgz
	rm -fr $(DOCUMENT)
	@echo "voila: $(DOCUMENT).tgz"

commit: clean 
	svn commit

count: $(DOCUMENT).pdf
	pdftotext $(DOCUMENT).pdf -|wc -w

update: clean 
	svn update


